No-Press Diplomacy from Scratch

Prior AI successes in complex games have largely focused on settings with at most hundreds of actions at each decision point. In contrast, Diplomacy is a game with more than 10^20 possible actions per turn. Previous attempts to address games with large branching factors, such as Diplomacy, StarCraft, and Dota, used human data to bootstrap the policy or used handcrafted reward shaping. In this paper, we describe an algorithm for action exploration and equilibrium approximation in games with combinatorial action spaces. This algorithm simultaneously performs value iteration while learning a policy proposal network. A double oracle step is used to explore additional actions to add to the policy proposals. At each state, the target state value and policy for the model training are computed via an equilibrium search procedure. Using this algorithm, we train an agent, DORA, completely from scratch for a popular two-player variant of Diplomacy and show that it achieves superhuman performance. Additionally, we extend our methods to full-scale no-press Diplomacy and for the first time train an agent from scratch with no human data. We present evidence that this agent plays a strategy that is incompatible with human-data bootstrapped agents. This presents the first strong evidence of multiple equilibria in Diplomacy and suggests that self play alone may be insufficient for achieving superhuman performance in Diplomacy.

==> sections/C_action_space.tex <==
\newpage
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/num_actions.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> sections/E_experiments.tex <==
\newpage
% \section{Comparison with DipNet Agents}
% \label{sec:compare_agents}

\section{Details on Experimental Setup}
\label{sec:experiments}

Most games on \url{webdiplomacy.net} were played with 24-hour turns, though the agent also played in some ``live'' games with 5-minute turns. Different hyperparameters were used for live games versus non-live games. In non-live games, we typically ran RM for 2,048 iterations with a rollout length of 3 movement phases, and set $M$ (the constant which is multiplied by the number of units to determine the number of subgame actions) equal to 5. This typically required about 20 minutes to compute. In live games (including games in which one human played against six bots) and in games against non-human opponents, we ran RM for 256 iterations with a rollout length of 2 movement phases, and set $M$ equal to 3.5. This typically required about 2 minutes to compute. In all cases, the temperature for the blueprint in rollouts was set to 0.75.


\begin{table*}[h!]
% \small
\begin{center}
\begin{tabular}{ l | c | c | c c c c }
\toprule
{\bf Power} & {\bf Score} & {\bf Human Mean} & {\bf Games} & {\bf Wins} & {\bf Draws} & {\bf Losses} \\
\midrule
% All Games & 26.8\% $\pm$ 4.5\% & 14.3\% & 64 & 10 & 21 & 33 \\
% Normalized By Power & 28.3\% $\pm$ 4.9\% & 14.3\% & 64 & 10 & 21 & 33 \\
% \midrule
% Austria & 35.8\% & 11.0\% & 9 & 2 & 3 & 4 \\
% England & 22.7\% & 12.6\% & 9 & 1 & 3 & 5 \\
% France & 8.6\% & 16.9\% & 11 & 0 & 4 & 7 \\
% Germany & 48.1\% & 15.0\% & 8 & 2 & 4 & 2 \\
% Italy & 40.5\% & 11.6\% & 7 & 2 & 3 & 2 \\
% Russia & 25\% & 14.8\% & 10 & 2 & 2 & 6 \\
% Turkey & 17.6\% & 18.2\% & 10 & 1 & 2 & 7 \\
All Games & 26.6\% $\pm$ 3.2\% & 14.3\% & 116 & 16 & 43 & 57 \\
Normalized By Power & 26.9\% $\pm$ 3.3\% & 14.3\% & 116 & 16 & 43 & 57 \\
\midrule
Austria & 31.4\% $\pm$ 9.4\% & 11.0\% & 17 & 3 & 6 & 8 \\
England & 38.0\% $\pm$ 10.1\% & 12.6\% & 16 & 4 & 6 & 6 \\
France & 19.0\% $\pm$ 6.2\% & 16.9\% & 19 & 1 & 8 & 10 \\
Germany & 36.8\% $\pm$ 8.0\% & 15.0\% & 16 & 2 & 10 & 4 \\
Italy & 31.5\% $\pm$ 10.5\% & 11.6\% & 14 & 3 & 5 & 6 \\
Russia & 17.6\% $\pm$ 7.6\% & 14.8\% & 18 & 2 & 4 & 12 \\
Turkey & 14.6\% $\pm$ 7.0\% & 18.2\% & 16 & 1 & 4 & 11 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\small Average SoS score of our agent in anonymous games against humans on \url{webdiplomacy.net}. Average human performance is 14.3\%. Score in the case of draws was determined by the rules of the joined game. The $\pm$ shows one standard error.
%Due to small sample sizes, we do not display a $\pm$ for individual powers.
Average human performance was calculated based on SoS scoring of historical games on \url{webdiplomacy.net}.
}
\label{tab:webdip2}
\end{table*}

\begin{table*}[h!]
% \small
\begin{center}
\begin{tabular}{ l | c c c }
\toprule
{\bf Power} & {\bf 1 Human vs. 6 DipNet} & {\bf 1 Human vs. 6 Blueprint} & {\bf 1 Human vs. 6 SearchBot} \\
\midrule
All Games & 39.1\% & 22.5\% & 5.7\% \\
\midrule
Austria & 40\% & 20\% & 0\% \\
England & 28.4\% & 20\% & 0\% \\
France & 20\% & 4.3\% & 40\% \\
Germany & 40\% & 33\% & 0\% \\
Italy & 60\% & 20\% & 0\% \\
Russia & 40\% & 20\% & 0\% \\
Turkey & 45.1\% & 40\% & 0\% \\
\bottomrule
\end{tabular}
\end{center}
\caption{\small Average SoS score of one expert human playing against six bots under repeated play. A score less than 14.3\% suggests the human is unable to exploit the bot. Five games were played for each power for each agent, for a total of 35 games per agent. For each power, the human first played all games against DipNet, then the blueprint model described in Section~\ref{sec:blueprint}, and then finally \botname{}.
}
\label{tab:human2}
\end{table*}

The experiments on \url{webdiplomacy.net} occurred over a three-month timespan, with games commonly taking one to two months to complete (players are typically given 24 hours to act). Freezing research and development over such a period would have been impractical, so our agent was not fixed for the entire time period. Instead, serious bugs were fixed, improvements to the algorithm were made, and the model was updated.

In games on \url{webdiplomacy.net}, a draw was submitted if \botname{} did not gain a center in two years, or if the agent's projected sum-of-squares score was less than the score it would achieve by an immediate draw. Since there was no way to submit draws through the \url{webdiplomacy.net} API, draws were submitted manually once the above criteria was satisfied. Games against other bots, shown in Table~\ref{tab:compare_agents}, automatically ended in a draw if no player won by 1935.

==> sections/F_observations.tex <==
\section{Qualitative Assessment of \botname{}}
\label{sec:observations}

\anton{I think we can add some comments from RJ here.}
